Understanding the Security of Deepfake Detection

Deepfakes pose growing challenges to the trust of information on the Internet. Thus, detecting deepfakes has attracted increasing attentions from both academia and industry. State-of-the-art deepfake detection methods consist of two key components, i.e., face extractor and face classifier, which extract the face region in an image and classify it to be real/fake, respectively. Existing studies mainly focused on improving the detection performance in non-adversarial settings, leaving security of deepfake detection in adversarial settings largely unexplored. In this work, we aim to bridge the gap. In particular, we perform a systematic measurement study to understand the security of the state-of-the-art deepfake detection methods in adversarial settings. We use two large-scale public deepfakes data sources including FaceForensics++ and Facebook Deepfake Detection Challenge, where the deepfakes are fake face images; and we train state-of-the-art deepfake detection methods. These detection methods can achieve 0.94--0.99 accuracies in non-adversarial settings on these datasets. However, our measurement results uncover multiple security limitations of the deepfake detection methods in adversarial settings. First, we find that an attacker can evade a face extractor, i.e., the face extractor fails to extract the correct face regions, via adding small Gaussian noise to its deepfake images. Second, we find that a face classifier trained using deepfakes generated by one method cannot detect deepfakes generated by another method, i.e., an attacker can evade detection via generating deepfakes using a new method. Third, we find that an attacker can leverage backdoor attacks developed by the adversarial machine learning community to evade a face classifier. Our results highlight that deepfake detection should consider the adversarial nature of the problem.

==> evaluation.tex <==
\section{Evaluation}
\subsection{Experimental settings}
\myparatight{Dataset} We consider two datasets, specifically the FaceForensics++ dataset [] and Facebook DeepFake Detection dataset []. FaceForensics++ dataset contains 1000 real videos from Youtube. Four face manipulation methods, specifically, DeepFakes, FaceSwap, Face2Face and NeuralTextures are used to generate fake videos based on the real videos, which results in 4,000 fake videos in total. We follow the original paper [] to split the real videos into training, validation and test sets, each containing 720,140 and 140 videos, respectively. If a fake video is generated from a real training (validation/testing) video, it will be considered as a training (validation/testing) video. We then extract face images using publicly available package Dlib[] from the videos for each frame, and resize it to $299\times299$. The face images extracted from training, validation and testing videos are used as training, validation and testing datasets, respectively. The Facebook DeepFake Detection dataset is a larger dataset consisting of videos sourced from 3,426 paid actors. The training set contains 19,154 ten-second real videos as well as 100,000 fake videos generated by multiple neural network-based manipulation methods, including DFAE, MM/NN face swap, NTH, FSGAN and StyleGAN. However, it is unknown that what method is used to generate each individual fake video. Therefore, we refer to the method that generate the dataset as a whole and call it Facebook. Since we do not have access to the private test set, we use 72\% of the training videos as training data, another 14\% as validataion data, and the rest 14\% as testing data. The same face extraction process as used for FaceForensics++ dataset will be applied to extract faces from the videos. However, to ensure that Facebook has roughly the same number of face images as other methods, we extract one face per 50 frames for fake videos and per 10 frames for real videos.


\myparatight{Training settings}  We follow [] to train Xception []  networks. Specifically, we initialize with the model pretrained on ImageNet. Then we train the model using Adam optimizer for 17 epochs, among which the first 2 only updates the last fully connected layer while the other 15 updates the entire model. The learning rate is set to 0.0002, the same as in []. For each of the five face manipulation methods, we train an Xception model using real faces and fake faces generated by the method as training data. We refer to the models as DF, FS, F2F, NT, and FB respectively. We also train another model that uses all face images as training data, which we denote by ALL.

\subsection{Experimental results}



\myparatight{Generalization to Gaussian random noise} We test the generalization to Gaussian noise of the five models, using the testing images that are generated by the same method as the training images. For instance, we use the testing images generated by DeepFakes to evaluate DF model. Gaussian noise with zero mean and different values of standard deviation is added to the testing images before fed into the models. Figure \ref{fig:noise} shows the accuracy, true positive rate (TPR), true negative rate (TNR) and AUC scores of different models. We ovbserve that all five models are not robust to Gaussian random noise. Specifically, when the standard deviation of the additive Gaussian noise is 0.03, the accuracy and AUC of all models drop to the level of random guessing. Another interesting finding is that the sum of TPR and TNR is close to 1 in all cases when the standard deviation is large. 
We suspect that this is because when the standard deviation is large, random noise becomes the dominating component when making an inference on the perturbed input. Therefore, we experiment on the label distribution of predictions made by different models on random Gaussian noise. Specifically, for each model, we sample 10,000 random Gaussian noise given a standard deviation and feed them into the model as inputs. We then compute the fraction of positive predictions and negative predictions among the outputs. Figure \ref{fig:random} show the results. We observe that when the standard deviation increases, the true positive rate tends to be the same as fraction of positives for random inputs while the true negative rate tends to be the same as fraction of negatives. We show some examples of perturbed inputs in Figure \ref{fig:noise_example}. 

We also consider the case when random gaussian noise is added directly to the video before the face extraction. Table \ref{fig:fe} shows the fraction of successful face extraction when $\sigma$ varies. We found that when the noise is large, it is hard for the face detector to successfully locate and extract the faces. 

\begin{figure*}[!t]
    \center
    \includegraphics[width=0.6\textwidth]{./figs/face_extraction.pdf}
    \caption{Fraction of successful face extraction when $\sigma$ varies.}
    \label{fig:fe}
\vspace{-3mm}
\end{figure*}







\myparatight{Generalization to unknown methods} We test the generalization to unknown methods of the four single-method models, i.e., DF, FS, F2F and NT. Table \ref{tab:unknown} shows the results. We find that the models cannot effectively generalize to unknown methods. For example, DF model has an accuracy of 0.99 and AUC score of 1 when inferring DeepFakes images. However, it only achieves 0.55 accuracy and 0.31 AUC when the testing images are generated by FaceSwap.

\myparatight{Generalization to adversarial perturbations} We consider two types of attacks, adversarial examples and poisoning attacks. For adversarial examples, we consider the popular FGSM method and PGD method. Figure \ref{fig:adv} shows the success rate of the attacks when the attack parameter $\epsilon$ is set to different values. We observe that with $\epsilon=0.001$, almost all attacks can achieve a success rate that is close to 1, which means that the models are sensitive to adversarial examples. Figure \ref{fig:adv_example} shows examples of adversarial examples against ALL model when attack parameter $\epsilon$ varies. 





We also explore two data poisoning attacks, specifically, label flipping attack and backdoor attack. For label flipping attack, we randomly flip labels of some training examples, i.e., if a video is real, we set its label to fake; if a video is fake, we set its label to real. The label of each training example will be fixed during the training process after the flip. The model will be trained with the poisoned dataset under the same training setting as when there is no attack. We evaluate the accuracy, true possitive rate, true negative rate and the AUC score of the trained models. Results can be found in Figure \ref{fig:all_lf}. We can observe that when the fraction of label-flipped data increases, the accuracy, false positive rate, false negative rate, and AUC score all decrease. However, when the fraction is either much smaller or larger than 0.5, the four numbers drop slowly; when the fraction is close to 0.5, there is a jump in them and the numbers drop from almost 1 to almost 0. This is intuitive as when there are more mislabeled data in the training set, the model is trained to make wrong predictions instead of correct ones. The results shows that the classifier is robust to label flipping attacks. 

For backdoor attack, we follow the BadNets attack \cite{} to use a black-and-white patch as a trigger. Specifically, we make copies of some training images and add the trigger to them. Figure \ref{fig:bd} shows the trigger and the images with the trigger added. We label the copies with the trigger as real images and add the (image, label) pairs to the training set. A backdoored model will be trained with the poisoned dataset following the same training process as the no-attack setting. Once the model with the backdoor is trained, we evaluate both the accuracy of the benign testing images and the backdoor accuracy of the attack. The backdoor accuracy is defined as the fraction of testing images with the trigger predicted as real images. Figure \ref{fig:all_bd} shows the performance of the attack when different fraction of training examples are poisoned. We observe that when the model is not backdoored, the trigger has no impact on the testing images and the backdoor accuracy is close to 0.5. However, when only 5\% of images with triggers are added into the training dataset, with their labels set to real,  the trained model with backdoor will achieve a backdoor accuracy as high as 1. This means that all testing images with the trigger will be predicted as real images by the backdoored model. The results indicate that the classifier is highly sensitive to backdoor attacks.






